Real-Time Face and Landmark Localization for Eyeblink Detection

Pavlovian eyeblink conditioning is a powerful experiment used in the field of neuroscience to measure multiple aspects of how we learn in our daily life. To track the movement of the eyelid during an experiment, researchers have traditionally made use of potentiometers or electromyography. More recently, the use of computer vision and image processing alleviated the need for these techniques but currently employed methods require human intervention and are not fast enough to enable real-time processing. In this work, a face- and landmark-detection algorithm have been carefully combined in order to provide fully automated eyelid tracking, and have further been accelerated to make the first crucial step towards online, closed-loop experiments. Such experiments have not been achieved so far and are expected to offer significant insights in the workings of neurological and psychiatric disorders. Based on an extensive literature search, various different algorithms for face detection and landmark detection have been analyzed and evaluated. Two algorithms were identified as most suitable for eyelid detection: the Histogram-of-Oriented-Gradients (HOG) algorithm for face detection and the Ensemble-of-Regression-Trees (ERT) algorithm for landmark detection. These two algorithms have been accelerated on GPU and CPU, achieving speedups of 1,753$\times$ and 11$\times$, respectively. To demonstrate the usefulness of our eyelid-detection algorithm, a research hypothesis was formed and a well-established neuroscientific experiment was employed: eyeblink detection. Our experimental evaluation reveals an overall application runtime of 0.533 ms per frame, which is 1,101$\times$ faster than the sequential implementation and well within the real-time requirements of eyeblink conditioning in humans, i.e. faster than 500 frames per second.

==> 0_template/ack.tex <==
% Thesis Acknowledgements ----------------------------------------------
%-----------------------------------------------------------------------%
%            Fixed part - Don't change any thing here                   %
%-----------------------------------------------------------------------%

%\begin{flushleft}
%\begin{Huge}{Acknowledgements}
%\end{Huge}
%\end{flushleft} \vskip 2cm

\nonumchapter{Acknowledgements}                        %{ACKNOWLEDGEMENTS}
\vskip 1cm

First and foremost, I would like to thank my thesis advisor, Christos Strydis of the Neuroscience department of Erasmus MC, for his guidance during the project and for always keeping the office lively and full of laughter. Furthermore, I would like to thank Zaid Al-Ars, my supervisor at Delft University of Technology, for helping me in the search for an interesting thesis topic and his valuable comments on this work. 

A big thank you also goes out to Henk-Jan Boele and Bas Koekkoek for the introduction into the fascinating world of neuroscience, George Smaragdos for his valuable comments on the thesis, Rene Miedema for his constant advice on every step of the implementation process, and everyone that participated in the eyeblink-conditioning experiments that were used for this thesis.  

Finally, I would like to express my gratitude to my parents, family, friends and Nienke, for their support throughout this project. This accomplishment would not have been possible without them. Thank you.



%-----------------------------------------------------------------------%
%     Please fill in your acknowledgements here                         %
%-----------------------------------------------------------------------%

%-----------------------------------------------------------------------%
%      no change here                                                    %
%-----------------------------------------------------------------------%

\vskip 2cm
\noindent \AUTHOR \\
\PLACE \\
\DATE



==> 0_template/acronym.tex <==
\chapter*{List of Acronyms}
\begin{acronym}
\acro{AFLW}{Annotated Facial Landmarks in the Wild}
\acro{API}{Application Programming Interface}
\acro{AVX}{Advanced Vector Extensions}
\acro{CNN}{Convolutional Neural Network}
\acro{CPU}{Central Processing Unit}
\acro{CR}{Conditioned Response}
\acro{CS}{Conditioned Stimulus}
\acro{DNN}{Deep Neural Network}
\acro{DoG}{Difference of Gaussian}
\acro{DPM}{Deformable Parts Model}
\acro{EMG}{Electromyography}
\acro{EOH}{Edge Orientation Histogram}
\acro{FLOPS}{Floating-point Operations Per Second}
\acro{FMA}{Fused Multiply-Add}
\acro{GPGPU}{General-Purpose computing on Graphics Processing Units}
\acro{GPU}{Graphics Processing Unit}
\acro{HOG}{Histogram of Oriented Gradients}
\acro{ICF}{Integral Channel Features}
\acro{LBP}{Local Binary Pattern}
\acro{LoG}{Laplacian of Gaussian}
\acro{NN}{Neural Network}
\acro{NVCC}{NVIDIA CUDA Compiler}
\acro{NVVP}{NVIDIA Visual Profiler}
\acro{OMP}{Open Multi-Processing}
\acro{OpenCV}{Open Source Computer Vision}
\acro{PCA}{Principal Component Analysis}
\acro{PCIe}{Peripheral Component Interconnect Express}
\acro{SDK}{Software Development Kit}
\acro{SIFT}{Scale-Invariant Feature Transform }
\acro{SIMD}{Singe Instruction Multiple Data}
\acro{SM}{Streaming Multiprocessor}
\acro{SMT}{Simultaneous Multithreading}
\acro{SURF}{Speeded-Up Robust Features}
\acro{SVR}{Support Vector Regression}
\acro{UR}{Unconditioned Response}
\acro{US}{Unconditioned Stimulus}
\acro{}{}
\end{acronym}

%MB GB ETC? KB

==> 0_template/cover.tex <==
% X. van Rijnsoever, 2014
% Frontpage with image
\AddToShipoutPicture*{
	\setlength{\unitlength}{1cm}
	\put( 0,  0){\includegraphics{figures/cover/TUDelft_border_back}}
    \put( 3,  1.7){\includegraphics{figures/cover/TUDelft_logo}}
    \put( 13,  1.7){\includegraphics[width=4.9cm]{figures/cover/celab_logo}}
	\put( 1, 13){\color{cyan}\linethickness{2cm}\line(0,1){7}}
	\put( 1, 14){\rotatebox{90}{\color{white}\large\textsf{Delft University of Technology}}}

    \definecolor{gray95}{gray}{0.95}
	\put( 2, 23){\color{gray95}\linethickness{6cm}\line(1,0){17}}
%	\put( 2.6, 24.7){\color{black}\linethickness{0.5mm}\line(0,-1){3.9}}

	\put( 3, 24){\color{black}{\Huge\textsf{Real-time Face and Landmark Localization}}}
	\put( 3, 23){\color{black}{\Huge\textsf{for Eyeblink-Response Detection}}}
	% \put( 3, 22){\color{black}{\Huge\textsf{}}}
	\put( 3, 21){\color{black}{\Large\textsf{Paul Bakker}}}
	\put( 14.5, 21){\color{black}{\Large\textsf{CE-MS-2017-16}}}
% Image:
%	\put( 4, 9.5){\includegraphics[width=13cm]{images/}}


\put( 3.5, 18.0){\color{black}\linethickness{0.5mm}\line(0,-1){10.5}}

}

\vspace*{7cm}
\noindent \Large\textsf{Abstract}

\bigskip

\noindent \normalsize \textsf{
Pavlovian eyeblink conditioning is a powerful experiment used in the field of neuroscience to measure multiple aspects of how we learn in our daily life. To track the movement of the eyelid during an experiment, researchers traditionally made use of potentiometers or electromyography (EMG). More recently, the use of computer vision and image processing alleviated the need for these techniques, but currently employed methods require human intervention and are not fast enough to enable real-time processing. %, which makes off-line storage of video data a necessity. 
We selected a combination of face and landmark-detection algorithms in order to fully automate eyelid tracking, and accelerated them to make the first step towards an on-line implementation. Various different algorithms for face detection and landmark detection (eyelid detection) are analyzed and evaluated. Based on this analysis, two algorithms are identified as most suitable for our use case: the Histogram of Oriented Gradients (HOG) algorithm for face detection and Ensemble of Regression Trees (ERT) algorithm for landmark detection. These two algorithms are accelerated on GPU and CPU, achieving speedups of 1753$\times$ and 11.49$\times$, respectively. A combination of these algorithms is successfully implemented for a real neuroscientific use-case: eyeblink response detection, achieving an overall application runtime of 0.533 ms per frame, which is 1101$\times$ faster than the sequential implementation. Furthermore, this accelerated implementation was used to generate a database of 1440 eyeblink responses during the conditioning experiment. We made use of multiple machine-learning techniques to analyze this database and concluded that there is a correlation between the asynchrony of the eyelids and the eyeblink-response performance during the conditioning experiment.}

~
\clearpage


==> 0_template/front.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                               %
%   Standard title page, no modifications required              %
%   Author: Wiebe Cnossen                                       %
%   Date:   August 11 1994                                      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Modified by Bao Linh Dang                                   %
%   Date: 15/4/2003                                             %
%   Modified by Ronald Bos: allow long TITLE                    %
%   Date: 5/4/2004                                              %
%   Put your abstract here(about 15 lines) and the rest should  %
%   not be changed !!!                                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-----------------------------------------------------------------------%
%            Fixed part - Don't change any thing here                   %
%-----------------------------------------------------------------------%
\thispagestyle{plain} \cleardoublepage

\topmargin -0.5in

% Ronald Bos: removed shortstack and some font size tweaking
% to allow a long TITLE (longer than one line)
\begin{center}
\huge \TITLE{} \\
\normalsize
\rule{5.5in}{1.5pt}
\vskip 0.5cm
by~\AUTHOR

\vskip 0.5cm {\bf Abstract}
\end{center}

% Start your abstract here 

\begin{small}
%------------------------------------------------------------------------%
%   Please fill in 
%       1) the first letter of the first word of your thesis abstract    %
%          into the first brace after \drop command                      %
%       2) the left letters of the first word of your thesis abstract    %
%          into the second brace                                         %
%       3) the left part of your thesis abstract after the second brace  %
%                                                                        %
%------------------------------------------------------------------------%
\
\input{0_template/abstract.tex}

\end{small}                                       % End of your abstract. 

% End of your abstract. The next part is fixed, don't change anything
%-----------------------------------------------------------------------%
%            Fixed part - Don't change any thing here                   %
%-----------------------------------------------------------------------%
\vskip 15pt
\begin{flushleft}
\begin{sloppypar}
\begin{tabular}{lll}
{\bf Laboratory }&:& \begin{minipage}[t]{9cm}
   {Computer Engineering}\end{minipage}    \\
{\bf Codenumber }&:& \NR         \\ \\
{\bf Committee Members }&:&
\end{tabular}
\end{sloppypar}
\end{flushleft}

\signaturepage \addtolength{\topmargin}{0.5in}
%\end{document}


==> references.tex <==
This thesis aims to employ current technologies to serve the neuroscientific effort, and is part of a larger collaboration between the Computer Engineering lab of Delft University of Technology and the Erasmus MC Neuroscience group. Other topics of this collaboration include:

\begin{itemize}
	\item Acceleration of large-scale brain simulations with various HPC node technologies such as FPGAs, GPUs, dataflow engines and many-core processors; 

	(H.A. Du Nguyen, Z. Al-Ars, G. Smaragdos, C. Strydis, "Accelerating Complex Brain-Model Simulations on GPU Platforms", 18th Design, Automation & Test in Europe conference (DATE 2015), 9-13 March 2015, Grenoble, France), 

	G Smaragdos, Z. Al-Ars, R. Kukreja, I. Sourdis, C. Kachris, D. Soudris, C. Strydis, BrainFrame: A node-level heterogeneous accelerator platform for neuron simulations (July 2017), Journal of Neural Engineering (J NEURAL ENG) [Journal Paper]

	\item Real-time whisker tracking for studying sensorimotor disorders;

	(Y. Ma, G Smaragdos, Z. Al-Ars, C. Strydis, "Towards Real-Time Whisker Tracking in Rodents for Studying Sensorimotor Disorders", International Conference on Embedded Computer Systems: Architectures, Modeling, and Simulation (SAMOS XVII), 17-20 July 2017, Samos, Greece)

	% \item Brain rescue and brain-machine interfaces;
	% \item Powerful, neuroscience-friendly modeling/simulation toolflow;
	% \item Improved neuronal recordings and feedback.
\end{itemize}


% Please strengthen the connection with the CE group and our collaboration with Erasmus MC by including more references in your thesis from our publications (http://www.ce.ewi.tudelft.nl/zaid/publications/). Here is a list you can include and integrate in the text.


% => J.J. Hoozemans, R.W. Heij, J. Van Straten, Z. Al-Ars, “VLIW-based FPGA Computational Fabric with Streaming Memory Hierarchy for Medical Imaging Applications", 13th International Symposium on Applied Reconfigurable Computing (ARC2017), 3-7 April 2017, Delft, The Netherlands
% => S. Ren, K.L.M. Bertels, Z. Al-Ars, "Exploration of Alternative GPU Implementations of the Pair-HMMs Forward Algorithm", 3rd International Workshop on High Performance Computing on Bioinformatics (HPCB 2016), 15-18 December 2016, Shenzhen, China
% => S. Ren, V.M. Sima, Z. Al-Ars, "FPGA Acceleration of the Pair-HMMs Forward Algorithm for DNA Sequence Analysis", International Workshop on High Performance Computing on Bioinformatics (HPCB 2015), 9-12 November 2015, Washington DC, USA
% => E.J. Houtgast, V.M. Sima, K.L.M. Bertels, Z. Al-Ars, "GPU-Accelerated BWA-MEM Genomic Mapping Algorithm Using Adaptive Load Balancing", 29th International Conference on Architecture of Computing Systems (ARCS 2016), 4-7 April 2016, Nuremberg, Germany 



% => Y. Ma, G Smaragdos, Z. Al-Ars, C. Strydis, "Towards Real-Time Whisker Tracking in Rodents for Studying Sensorimotor Disorders", International Conference on Embedded Computer Systems: Architectures, Modeling, and Simulation (SAMOS XVII), 17-20 July 2017, Samos, Greece
% => H.A. Du Nguyen, Z. Al-Ars, G. Smaragdos, C. Strydis, "Accelerating Complex Brain-Model Simulations on GPU Platforms", 18th Design, Automation & Test in Europe conference (DATE 2015), 9-13 March 2015, Grenoble, France
% => G Smaragdos, Z. Al-Ars, R. Kukreja, I. Sourdis, C. Kachris, D. Soudris, C. Strydis, "BrainFrame: A Node-Level Heterogeneous Accelerator Platform for Neuron Simulations", Journal of Neural Engineering (J NEURAL ENG), 2017
